Tips and Tricks in linear imaging polarimetry of extended sources with FORS2 at the VLT

Context: Polarimetry is a very powerful tool to uncover various properties of astronomical objects that remain otherwise hidden in standard imaging or spectroscopic observations. However, the reliable measurement of the low polarization signal from astronomical sources requires a good control of spurious instrumental polarization induced by the various components of the optical system and the detector. Aims: We perform a detailed multi-wavelength calibration study of the FORS2 instrument at the VLT operating in imaging polarimetric mode (IPOL) to characterize the spatial instrumental polarization that may affect the study of extended sources. Methods: We use imaging polarimetry of a) high signal-to-noise blank fields BVRI observations during full-moon, when the polarization is expected to be constant across the field-of-view and deviations originate from the instrument and b) a crowded star cluster in broad-band RI and narrow-band H{\alpha} filters, where individual polarization values of each star across the field can be measured. Results: We find an instrumental polarization pattern that increases radially outwards from the optical axis of the instrument reaching up to 1.4% at the edges, depending on the filter. Our results are well approximated by an elliptical paraboloid down to less than {\sim0.05\%} accuracy,and {\sim0.02\%} when using non-analytic fits. We present 2D maps to correct for this spurious instrumental polarization. We also give several tips and tricks to analyze polarimetric measurements of extended sources. Conclusions: FORS2 is a powerful instrument allowing to map the linear polarimetry of extended sources. We present and discuss a methodology to measure the polarization of such sources, and to correct for the spatial polarization induced in the optical system. This methodology could be applied to polarimetric measurements using other dual-beam polarimeters.

==> ap_inla.tex <==
In this section, we use a non-analytic fitting procedure to obtain maps of Stokes parameters, $Q$ and $U$, the polarization degree, $P$, and angle, $\chi$, of the FORS2 instrument optics in $BVRI$ obtained from the same moonlit blank fields investigated in section~\ref{sec:instpol_moon}. In principle, this allows for a reconstruction that is less subject to forced features from the assumed analytic function. We use a method that is based on Gaussian Markov Random Fields, which model the underlying continuous spatial field with hyper-parameters fitted with a Bayesian inference algorithm known as Integrated Nested Laplace Approximation \citep[INLA,][]{Rue17}. The method has been successfully applied in many different areas including extended sources in astronomy \citep{Gonzalez19}. It offers the additional advantage of full posterior distributions to properly model uncertainties. 

We show in Figure~\ref{fig:QUinla} the reconstruction of $Q$ and $U$ for the $B$-band to be compared with the analytic fits of Figure~\ref{fig:QU}. Although at first the INLA maps look quite similar to the analytic hyperbolic paraboloid, the residuals are at least one order of magnitude smaller and show no clear patterns, as opposed to the analytic fits. The advantage of the INLA fits becomes more evident in the polarization degree fits shown in Figure~\ref{fig:polinla}, where the asymmetric behaviour is clearly visible in the reconstruction and it is confirmed in the rather flat residual map. We present the median and deviation of all residual maps in Table~\ref{table:resinla}. We also release all final INLA reconstructions \href{https://baltasar.tecnico.ulisboa.pt/~sgonzalez/FORS2-INSTPOL/}{here}.


\begin{figure*}
\includegraphics[trim={1.4cm 1.5cm 1.2cm 1.5cm },clip,width=0.49\textwidth]{Figures/b_HIGH-bin15pix2sig-corrmed-Qinla.png}
\includegraphics[trim={1.4cm 1.5cm 1.2cm 1.5cm },clip,width=0.49\textwidth]{Figures/b_HIGH-bin15pix2sig-corrmed-Uinla.png}
\caption{\label{fig:QUinla} \emph{Top}: Binned Q (left) and U (right) maps in $B$-band. \emph{Middle}: Non-analytic INLA 2D fit. \emph{Bottom}: Residual of observed map minus the fit.}
\end{figure*}

\begin{figure*}
\includegraphics[trim={1.4cm 1.5cm 1.2cm 1.5cm },clip,width=0.49\textwidth]{Figures/v_HIGH-bin15pix2sig-corrmed-polinla.png}
\includegraphics[trim={1.4cm 1.5cm 1.2cm 1.5cm },clip,width=0.49\textwidth]{Figures/I_BESS-bin15pix2sig-corrmed-polinla.png}
\caption{\label{fig:polinla} Binned polarization map (top), INLA fit (middle) and residual between the two (bottom) for filters $V$ (left) and $I$ (right) of moonlit sky.}
\end{figure*}

\begin{table*}[h!t]
\centering
% \scalebox{0.7}{
\begin{threeparttable}
 \caption{Median and median absolute deviation of the residual maps for the INLA fits of $Q$, $U$, $P$ and $\chi$.}\label{table:resinla}
 \begin{tabular}{c|cccc}
    \hline
\hline  
Filter & $B$-band & $V$-band & $R$-band & $I$-band\\
\hline
<Res(Q) [$10^{-2}$\%]> & 0.027$\pm$1.500 & 0.159$\pm$1.460 & 0.037$\pm$1.419 & 0.017$\pm$1.337 \\
<Res(U) [$10^{-2}$\%]> & -0.096$\pm$1.454 & -0.147$\pm$1.626 & -0.032$\pm$1.528 & -0.056$\pm$1.363 \\
<Res(P) [$10^{-2}$\%]>$^{\Diamond}$ & 0.018$\pm$1.514 & -0.654$\pm$1.652 & -0.003$\pm$1.531 & 0.026$\pm$1.396 \\
<Res($\chi$) [$10^{-1}$ deg]> & 0.116$\pm$8.455 & 0.337$\pm$6.650 & 0.240$\pm$4.776 & 0.284$\pm$5.678 \\
    \end{tabular}
    \begin{tablenotes}
      \small
      \item[$\Diamond$] These median polarization degree residuals correspond to 0.003$\sigma_B$, -0.040$\sigma_V$, -0.001$\sigma_R$ and 0.012$\sigma_I$ for $BVRI$ respectively, where $\sigma$ is the median error of each filter from Table~\ref{table:error}.
    \end{tablenotes}
\end{threeparttable}
%}
\end{table*}

